ZK-eSIM: A Privacy-Centric Zero-Knowledge Approach for eSIM Provisioning

GSMA Remote SIM Provisioning (RSP) enables over-the-air delivery of eSIM profiles, but it exposes long-lived identifiers during profile ordering and download. In particular, stable device identifiers (e.g., EID), profile identifiers, and long-lived certificate material enable mobile operators and profile-delivery infrastructure to link provisioning events to the same eUICC and, when combined with account records, to the same subscriber. This undermines subscriber anonymity and enables cross-session tracking. We present ZK-eSIM, a privacy-preserving redesign that achieves subscriber anonymity and provisioning-session unlinkability while retaining accountable traceability by exception. ZK-eSIM (i) replaces direct disclosure of device identifiers with a zero-knowledge proof of device validity and eligibility; (ii) enforces session unlinkability through short-lived, one-time pseudonymous credentials and per-session identifiers to prevent cross-session tracking; and (iii) provides privacy-preserving accountable traceability through a jointly authorised escrow mechanism, so that no single entity can unilaterally deanonymise a user. We formalise a multi-entity, honest-but-curious threat model and prove subscriber anonymity and the unlinkability of provisioning sessions under standard cryptographic assumptions. We implement a Java Card applet on a test eUICC to evaluate performance on commodity hardware with a modified LPA and SM-DP+ server. Our experiments quantify end-to-end cryptographic overhead relative to conventional RSP, confirming that ZK-eSIM adds only practical overhead, closing a critical privacy gap while preserving deployability within existing GSMA roles and interfaces.

==> old/OldPrivacyRisks.tex <==
% Assumes you already defined TikZ styles like:
%   role, lifeline, msgbox, setupmini, blackcap
% and you have \step{..} + (optional) fontawesome icons if you use them.
% Also add in your preamble (once): \usetikzlibrary{decorations.pathreplacing}

\begin{tikzpicture}[x=1pt,y=1pt]

  %========================
  % Column x-positions
  %========================
  \def\xA{0}    % Device A
  \def\xB{75}   % Device B
  \def\xMNOA{142}% MNO/MVNO A
  \def\xMNOB{205}% MNO/MVNO B
  \def\xSMDP{270}% SM-DP+

  \def\topY{230}
  \def\botY{-400}

  %========================
  % Derived coordinates (FIX: avoid inline arithmetic in coords)
  %========================
  \pgfmathsetmacro{\xTitle}{0.5*(\xA+\xSMDP)}
  \pgfmathsetmacro{\yTitle}{\topY+26}
  \pgfmathsetmacro{\xCompose}{0.5*(\xMNOA+\xSMDP)}

  %========================
  % Headers
  %========================
  \node[role, fill=partyblue, minimum width=30pt] (DevA) at (\xA,\topY)
    {\textbf{Device A} \faIcon{mobile-alt}\\\textbf{UE/LPA}\\\textbf{ eUICC}};
  \node[role, fill=partyblue, minimum width=30pt] (DevB) at (\xB,\topY)
    {\textbf{Device B} \faIcon{clock}\\\textbf{UE/LPA}\\\textbf{eUICC}};
  \node[role, fill=orange!30, minimum width=30pt] (MNOA) at (\xMNOA,\topY)
    {\textbf{MNO\textbackslash}\\\textbf{MVNO 1}};
  \node[role, fill=partygreen, minimum width=30pt] (MNOB) at (\xMNOB,\topY)
    {\textbf{MNO\textbackslash}\\\textbf{MVNO 2}};

  % SM-DP+ (boxed / shared)
  \node[role, fill=white, draw=black, rounded corners=2pt, minimum width=30pt] (SMDP) at (\xSMDP,\topY)
    {\textbf{SM-DP+}\\{\footnotesize (multi-tenant)}};

  %========================
  % Same subscriber brace (Option 1)
  %========================
  \pgfmathsetmacro{\yOwner}{\topY+20} % tweak vertical placement if needed
  \draw[decorate, decoration={brace, amplitude=4pt}, line width=0.6pt]
    (\xA-30, \yOwner) -- (\xB+30, \yOwner)
    node[midway, yshift=0pt, font=\small\bfseries]{Same subscriber (same user)};

  %========================
  % Lifelines
  %========================
  \draw[lifeline] (\xA,\topY-+18) -- (\xA,\botY-35);
  \draw[lifeline] (\xB,\topY-+18) -- (\xB,\botY-35);
  \draw[lifeline] (\xMNOA,\topY-+12) -- (\xMNOA,\botY-35);
  \draw[lifeline] (\xMNOB,\topY-+12) -- (\xMNOB,\botY-35);
  \draw[lifeline] (\xSMDP,\topY-+12) -- (\xSMDP,\botY-35);

  % bottom caps
  \node[blackcap] at (\xA,\botY-35) {};
  \node[blackcap] at (\xB,\botY-35) {};
  \node[blackcap] at (\xMNOA,\botY-35) {};
  \node[blackcap] at (\xMNOB,\botY-35) {};
  \node[blackcap] at (\xSMDP,\botY-35) {};



  \def\yPhaseZero{210}
  \node[font=\bfseries, anchor=west, fill=white] at (\xA-35
  ,\yPhaseZero-6) {Phase 0 (Pre-RSP): Intent / Contract Subscription};

  \def\yA0{180}
  
  \def\yB0{80}
\draw[dashed,
      rounded corners=6pt,
      line width=0.8pt, draw=red]
  (\xA-30,\yA0+6) rectangle (\xMNOA+40,\yB0+26);

\node[anchor=north west, font=\small\bfseries, text=red!70!black, fill=white]
  at (\xA-35,\yA0+20){R1: Identity–EID binding at subscription time};

%   \node[
%   draw=black,
%   fill=yellow!20,
%   rounded corners=3pt,
%   font=\scriptsize,
%   text width=50pt,
%   align=left
% ] at (\xMNOA+95,\yA0-10)
% {R1 links multiple devices to the same real-world user};

\draw[->, line width=0.6pt]
  (\xA,\yA0-8) -- ++(25,0)
  node[pos=0.4, above, font=\small] {\step{1} GetEID}
  -- ++(0,-3) -- ++(-25,0);

  \draw[->, line width=0.6pt] (\xA,\yA0-33) -- (\xMNOA,\yA0-33)
    node[midway, above, font=\small, text width=210pt, align=center]{%
          \step{2} \textit{Contract subscription}
      {\footnotesize Operator acquires:
      \textcolor{red}{identity},
      \textcolor{red}{billing},
      \textcolor{red}{EID\textsubscript{A}}, profileType)}
    };

 

\draw[->, line width=0.6pt]
  (\xB,\yB0+54)  -- ++(25,0)
  node[pos=0.4, above, font=\small] {\step{3} GetEID}
  -- ++(0,-3) -- ++(-25,0);

  \draw[->, line width=0.6pt] (\xB,\yB0+29) -- (\xMNOA,\yB0+29)
    node[midway, above, font=\small, text width=210pt, align=center]{%
      \step{4} \textit{Contract subscription}
      {\footnotesize Operator acquires:
      \textcolor{red}{identity},
      \textcolor{red}{billing},
      \textcolor{red}{EID\textsubscript{B}}, profileType)}
    };


  \def\yPhaseES9{10}
  \node[font=\bfseries, anchor=west, fill=white, text width=350pt] at (\xA-35,\yPhaseES9+82) {Profile Provisioning Sessions: Session 1 at Destination X (5-18), Session 2 at Destination Y (19-32)};

  \def\ytOne{-25}
  \def\ytTwo{-205}
   \node[anchor=north west, font=\small\bfseries, text=red!70!black, fill=white]
   at (\xA-35,\ytOne+107)
   {R2: Cross-session / cross-operator linking (SM-DP+ join point)};
 \draw[dashed,
       rounded corners=6pt,
       line width=0.9pt,
       draw=red]
  (\xA-30,\ytOne+95) rectangle (\xSMDP+45,\ytTwo-225);

% \node[
%   draw=black,
%   fill=yellow!20,
%   rounded corners=3pt,
%   font=\scriptsize,
%   text width=50pt,
%   align=left
% ] at (\xSMDP-235,\ytOne+50)
% {Same EID reused across provisioning sessions enables cross-operator linking};
 

\draw[->, line width=0.6pt] (\xMNOA,\ytOne+79) -- (\xSMDP,\ytOne+79)
  node[midway, above, font=\small, text width=210pt, align=center]{%
    \step{5} DownloadOrder(\textcolor{red}{EID\textsubscript{A}}, profileType=X)
  };

\node[msgbox, anchor=west, text width=75pt, align=center, inner sep=2pt] at (\xSMDP-50,\ytOne+69) {%
  \step{6} Reserve \textcolor{red}{ICCID\textsubscript{1}}
};

\draw[->, line width=0.6pt] (\xSMDP,\ytOne+49) -- (\xMNOA,\ytOne+49)
  node[midway, above, font=\small]{\step{7} \textcolor{red}{ICCID\textsubscript{1}}, MatchingID};

\draw[<-, line width=0.6pt] (\xSMDP,\ytOne+34) -- (\xMNOA,\ytOne+34)
  node[midway, above, font=\small]{\step{8} ConfirmOrder(\textcolor{red}{ICCID\textsubscript{1}},\textcolor{red}{EID\textsubscript{A}},releaseFlag=true)};

\node[msgbox, anchor=west, text width=70pt, align=center, inner sep=2pt] at (\xSMDP-50,\ytOne+19) {%
  \step{9} Map \textcolor{red}{ICCID\textsubscript{1} $\leftrightarrow$ EID\textsubscript{A}}
};
  \draw[->, line width=0.6pt] (\xMNOA,\ytOne+9) -- (\xA,\ytOne+9)
    node[midway, above, font=\small]{\step{10}\textit{Deliver Activation Code} {\footnotesize (SM-DP+ addr, AC Token)}};


    
 \def\yChal{-105}
\draw[->, line width=0.6pt]
    (\xA, \yChal+73) -- ++(25,0)
    node[above, font=\small, text width=460pt, align=left]{%
      \hspace{+180pt}\step{11} GetEUICCInfo, GetEUICCChallenge\\
      
    }  -- ++(0,-3) -- ++(-25,0);


  \draw[->, line width=0.6pt] (\xA,\ytOne-24) -- (\xSMDP,\ytOne-24)
    node[midway, above, font=\small, text width=300pt, align=center]{%
      \step{12} InitiateAuthentication(euiccChallenge,
      euiccInfo1,
      smdpAddress, ...)
    };

 

 \def\ySA{-155}
  \draw[->, line width=0.6pt] (\xSMDP, \ySA+92) -- (\xA, \ySA+92)
    node[midway, above, font=\small, text width=300pt, align=center]{%
      \step{13} transactionId\textsubscript{1},\;serverSigned1,\;serverSignature1,\;%
      CERT.DPauth.SIG%
    };

     \def\yAS{-180}
  \draw[->, line width=0.6pt]
    (\xA, \yAS+95) -- ++(25,0)
    node[above, font=\small, text width=180pt, align=left]{%
      \hspace{+40pt}\step{14} AuthenticateServer(...)\\
      {\hspace{+55pt}\footnotesize eUICC verifies SM-DP+}\\
    }
    -- ++(0,-3) -- ++(-25,0);


\node[font=\small\bfseries, text=red!70!black, fill=white]
  at (\xA+26, \yAS+82) {R3: Cert-chain fingerprint};


%    \node[
%   draw=black,
%   fill=yellow!20,
%   rounded corners=3pt,
%   font=\scriptsize,
%   text width=60pt,
%   align=left
% ] at (\xSMDP-235,\ytOne-135)
% {Static eUICC certificate reveals persistent device identity};
   
 \draw[dashed, rounded corners=5pt, line width=0.9pt, draw=red]
   (\xA-20,   \ytOne-78) rectangle (\xSMDP+40, \ytOne-140);
   
  \def\yACl{-140}
  \draw[->, line width=0.6pt] (\xA, \yACl+12) -- (\xSMDP, \yACl+12)
    node[midway, above, font=\small, text width=310pt, align=center]{%
      \step{15} AuthenticateClient(euiccSigned1,\;euiccSignature1,\\
      \textcolor{red}{CERT.EUICC.SIG\;(contains EID\textsubscript{A})},\;%
      CERT.EUM.SIG)%
    };

\node[msgbox, anchor=west, text width=70pt, align=center, inner sep=2pt] at (\xSMDP-50,\ytOne-122) {%
  \step{16} Verify eUICC cert chain;
  persist \textcolor{red}{EID\textsubscript{A}}
  $\leftrightarrow$ ICCID\textsubscript{1}%
};

\draw[->, line width=0.6pt] (\xSMDP,\ytOne-155) -- (\xA,\ytOne-155)
  node[midway, above, font=\small]{\step{17} Profile download\;\&\;install (ICCID\textsubscript{1})%
  };

\def\ysTwo{-355}


  
\draw[->, line width=0.6pt] (\xMNOB,\ysTwo+159) -- (\xSMDP,\ysTwo+159)
  node[midway, above, font=\small, text width=210pt, align=center]{%
    \hspace{-45pt}\step{18} DownloadOrder(\textcolor{red}{EID\textsubscript{A}}, profileType=Y)
  };

\node[msgbox, anchor=west, text width=70pt, align=center, inner sep=2pt] at (\xSMDP-50,\ysTwo+149) {%
  \step{19} Reserve \textcolor{red}{ICCID\textsubscript{2}}
};

\draw[->, line width=0.6pt] (\xSMDP,\ysTwo+129) -- (\xMNOB,\ysTwo+129)
  node[midway, above, font=\small]{\step{20} \textcolor{red}{ICCID\textsubscript{2}}, MatchingID};

\draw[<-, line width=0.6pt] (\xSMDP,\ysTwo+115) -- (\xMNOB,\ysTwo+115)
  node[midway, above, font=\small]{\hspace{-55pt}\step{21} ConfirmOrder(\textcolor{red}{ICCID\textsubscript{2}},\textcolor{red}{EID\textsubscript{A}},releaseFlag=true)};


\node[msgbox, anchor=west, text width=70pt, align=center, inner sep=2pt] at (\xSMDP-50,\ysTwo+100) {%
  \step{22} Map \textcolor{red}{ICCID\textsubscript{2} $\leftrightarrow$ EID\textsubscript{A}}
};

\draw[->, line width=0.6pt] (\xMNOB,\ysTwo+90) -- (\xA,\ysTwo+90)
  node[midway, above, font=\small]{\step{23} \textit{Deliver Activation Code} {\footnotesize (SM-DP+ addr, AC Token)}};

\def\yChalTwo{-435}
\draw[->, line width=0.6pt]
  (\xA, \yChalTwo+155) -- ++(25,0)
  node[above, font=\small, text width=360pt, align=left]{%
    \hspace{+130pt}\step{24} GetEUICCInfo, GetEUICCChallenge\\
  } -- ++(0,-3) -- ++(-25,0);

\draw[->, line width=0.6pt] (\xA,\ysTwo+58) -- (\xSMDP,\ysTwo+58)
  node[midway, above, font=\small, text width=240pt, align=center]{%
    \step{25} InitiateAuthentication(euiccChallenge,
    euiccInfo1,
    smdpAddress, ...)
  };
\def\ySATwo{-485}
\draw[->, line width=0.6pt] (\xSMDP, \ySATwo+174) -- (\xA, \ySATwo+174)
  node[midway, above, font=\small, text width=300pt, align=center]{%
    \step{26} transactionId\textsubscript{2},\;serverSigned1,\;serverSignature1,\;%
    CERT.DPauth.SIG%
  };

\def\yASTwo{-510}
\draw[->, line width=0.6pt]
  (\xA, \yASTwo+178) -- ++(25,0)
  node[above, font=\small, text width=180pt, align=left]{%
    \hspace{+40pt}\step{27} AuthenticateServer(...)\\
    {\hspace{+55pt}\footnotesize eUICC verifies SM-DP+}\\
  }
  -- ++(0,-3) -- ++(-25,0);

\node[font=\small\bfseries, text=red!70!black, fill=white]
  at (\xA+26, \ysTwo+10) {R3: Cert-chain fingerprint};

\draw[dashed, rounded corners=5pt, line width=0.9pt, draw=red]
  (\xA-20, \ysTwo+5) rectangle (\xSMDP+40, \ysTwo-58);

\def\yAClTwo{-420}
\draw[->, line width=0.6pt] (\xA, \yAClTwo+47) -- (\xSMDP, \yAClTwo+47)
  node[midway, above, font=\small, text width=310pt, align=center]{%
    \step{28} AuthenticateClient(euiccSigned1,\;euiccSignature1,\\
    \textcolor{red}{CERT.EUICC.SIG\;(contains EID\textsubscript{A})},\;%
    CERT.EUM.SIG)%
  };

\node[msgbox, anchor=west, text width=70pt, align=center, inner sep=2pt] at (\xSMDP-50,\ysTwo-38) {%
  \step{29} Verify eUICC cert chain;
  persist \textcolor{red}{EID\textsubscript{A}}
  $\leftrightarrow$ ICCID\textsubscript{2}%
};

\draw[->, line width=0.6pt] (\xSMDP,\ysTwo-71) -- (\xA,\ysTwo-71)
  node[midway, above, font=\small]{\step{30} Profile download\;\&\;install (ICCID\textsubscript{2})%
  };

%   \draw[->, line width=0.6pt] (\xSMDP,\ytOne-90) -- (\xA,\ytOne-90)
%     node[midway, above, font=\small]{\step{12}\; transactionId\textsubscript{1}, serverChallenge\textsubscript{1}};


%   % DevA -> SMDP AuthenticateClient with euiccCertChain
%   \draw[->, line width=0.6pt] (\xA,\ytOne-135) -- (\xSMDP,\ytOne-135)
%     node[midway, above, font=\small, text width=265pt, align=center]{%
%       \step{13}\; ES9+.AuthenticateClient(transactionId\textsubscript{1}, \dots, euiccCertChain\{\textcolor{red}{Cert\textsubscript{eUICC}}, \dots\})
%     };


%   \draw[->, line width=0.6pt] (\xSMDP,\ytOne-155) -- (\xA,\ytOne-155)
%     node[midway, above, font=\small]{\step{14}\; Download \& install profile (ICCID\textsubscript{A1})};

 
%   \draw[->, line width=0.6pt] (\xA,\ytTwo+10) -- (\xMNOB,\ytTwo+10)
%     node[midway, above, font=\small]{\step{15} User purchases plan ``Destination Y''};

% \draw[->, line width=0.6pt] (\xMNOB,\ytTwo-10) -- (\xSMDP,\ytTwo-10)
%   node[midway, above, font=\small, text width=210pt, align=center]{%
%     \step{16}ES2+.DownloadOrder(\textcolor{red}{EID\_A}, profileType=Y)
%   };

% \node[msgbox, anchor=west, text width=75pt, align=center] at (\xSMDP-45,\ytTwo-24) {%
%   \step{17} Reserve \textcolor{red}{ICCID\textsubscript{2}}
% };

%   \draw[->, line width=0.6pt] (\xSMDP,\ytTwo-50) -- (\xMNOB,\ytTwo-50)
%     node[midway, above, font=\small]{\step{18} \textcolor{red}{ICCID\textsubscript{2}}};

%     \draw[<-, line width=0.6pt] (\xSMDP,\ytTwo-70) -- (\xMNOB,\ytTwo-70)
%   node[midway, above, font=\small]{\step{19} ES2+.ConfirmOrder(\textcolor{red}{ICCID\textsubscript{2}},\textcolor{red}{EID\_A},releaseFlag)};

%   \draw[->, line width=0.6pt] (\xMNOB,\ytTwo-75) -- (\xA,\ytTwo-75)
%     node[midway, above, font=\small]{\step{19}\; Deliver activation\_code\textsubscript{2}, SMP-DP+ address};


%   \draw[->, line width=0.6pt] (\xA,\ytTwo-105) -- (\xSMDP,\ytTwo-105)
%     node[midway, above, font=\small, text width=240pt, align=center]{%
%       \step{20}\; ES9+.InitiateAuthentication(\textcolor{red}{EID\textsubscript{A}}, activation\_code\textsubscript{B1}, tenant=B)
%     };

% \draw[->, line width=0.6pt]
%   (\xSMDP,\ytTwo-140) -- ++(30,0)
%   node[above, font=\small, text width=210pt, align=left]{%
%     \step{21}\; Persist\\
%     \textcolor{red}{EID\textsubscript{A}} $\leftrightarrow$ ICCID\textsubscript{B1}\\
%     (tenant=B)
%   }
%   -- ++(0,-10)
%   -- (\xSMDP,\ytTwo-150);
 
%   \draw[->, line width=0.6pt] (\xSMDP,\ytTwo-155) -- (\xA,\ytTwo-155)
%     node[midway, above, font=\small]{\step{22}\; transactionId\textsubscript{2}, serverChallenge\textsubscript{2}};

 % \draw[dashed, rounded corners=5pt, line width=0.9pt, draw=red]
 %   (\xA-20,   \ytTwo-160) rectangle (\xSMDP+20, \ytTwo-190);

 % \node[ font=\small\bfseries, text=red!70!black, fill=white]
 %   at (\xA+27, \ytTwo-135) {R3: Cert-chain fingerprint};   \draw[->, line width=0.6pt] (\xA,\ytTwo-185) -- (\xSMDP,\ytTwo-185)
%     node[midway, above, font=\small, text width=270pt, align=center]{%
%       \step{23}\; ES9+.AuthenticateClient(transactionId\textsubscript{2}, \dots, euiccCertChain\{\textcolor{red}{same Cert\textsubscript{eUICC}}, \dots\})
%     };

%   \draw[->, line width=0.6pt] (\xSMDP,\ytTwo-210) -- (\xA,\ytTwo-210)
%     node[midway, above, font=\small]{\step{24}\; Download \& install profile (ICCID\textsubscript{B1})};


\end{tikzpicture}

==> uml/Mutual_Authentication.tex <==
@startuml
skinparam monochrome true
skinparam sequenceMessageAlign center
skinparam participantPadding 20
skinparam NoteBackgroundColor #F8F8F8
hide footbox

title Mutual Authentication in RSP

participant "SM-DP+ server (S)" as S
participant "LPA, User" as LPA
participant "eUICC (U)" as U

== Mutual Authentication ==

LPA -> U : 1. GetChallenge
U -> U: N_U := R

U -> LPA : 2.N_U,\n SKI_CI


LPA <-> S : HTTPS tunnel to S with Cert_St

LPA -> LPA: Cert_St ⊳ Cert_CI

S <- LPA : 3. N_U, S, SKI_CI\n

S -> S: S = subject of Cert_St\nI_t := R, N_S := R

S -> LPA : 4. Cert_Sa,\nSign(I_t, N_S, N_U, S; SK_Sa)

LPA -> LPA : Check that same S returned,\n[expected serverOID in Cert_Sa]
LPA -> U : 5. Cert_Sa, Iac,\nSign(I_t, N_S, N_U, S; SK_Sa)
U -> U: Cert_Sa ⊳ Cert_CI\n

U -> LPA : 6. PCert_U, Cert_EUM,\nSign(I_t, N_S, S, Iac; SK_U)

LPA -> S : 6. PCert_U, Cert_EUM,\nSign(I_t, N_S, S, Iac; SK_U)


note left
PCert_U ⊳ Cert_EUM,\nCert_EUM ⊳ Cert_CI
[Iac = Iac^expected],\n[U = subject of PCert_U]
event S1
end note

@enduml


==> uml/Profile_Download_Initiation <==
O -> U :  ConfirmRequest(H(pid)), pid \n (enc. under U’s PK)

@startuml
hide footbox
skinparam sequenceMessageAlign center
skinparam sequenceArrowFontSize 11
skinparam noteFontSize 11
skinparam monochrome true
skinparam lifelineStrategy solid

participant "User Device (U)" as U
participant "MNO (O)" as O
participant "MVNO (B)" as B
participant "SM-DP+" as DP


U -> O : ZKP, EncryptedRequest(eid) \n (enc. under B’s PK)


O -> B : ZKP, EncryptedRequest(eid) \n (enc. under B’s PK)

B -> B : verify ZKP

B -> B : generate $pid$

note right of B
  Computes H(pid).
end note

B -> DP : DownloadOrder(H($pid$), ProfileType)

DP -> DP : Allocate ICCID \n Bind to H($pid$)
DP --> B : Confirm
B -> DP : ConfirmOrder(releaseFlag)
DP --> B : H(pid)


B -> O : ConfirmRequest(H(pid)), pid \n (enc. under U’s PK), BBS+ Credential on (EID, PID)


O -> U :  ConfirmRequest(H(pid)), pid \n (enc. under U’s PK), BBS+ Credential on (EID, PID)



@enduml

